FIT: A Metric for Model Sensitivity

Model compression is vital to the deployment of deep learning on edge devices. Low precision representations, achieved via quantization of weights and activations, can reduce inference time and memory requirements. However, quantifying and predicting the response of a model to the changes associated with this procedure remains challenging. This response is non-linear and heterogeneous throughout the network. Understanding which groups of parameters and activations are more sensitive to quantization than others is a critical stage in maximizing efficiency. For this purpose, we propose FIT. Motivated by an information geometric perspective, FIT combines the Fisher information with a model of quantization. We find that FIT can estimate the final performance of a network without retraining. FIT effectively fuses contributions from both parameter and activation quantization into a single metric. Additionally, FIT is fast to compute when compared to existing methods, demonstrating favourable convergence properties. These properties are validated experimentally across hundreds of quantization configurations, with a focus on layer-wise mixed-precision quantization.

==> macros_general.tex <==



%----------------------------------------------------------------
\topmargin     0.0cm
\oddsidemargin -0.1cm %-0.1cm
\textwidth     16.8cm%16.8cm
\headheight    0.0cm
\textheight    22.2cm
\parindent     6mm
\parskip       1pt
\tolerance     1000


%----------------------------------------------------------------




%\declaretheorem[name=Theorem,numberlike=theorem]{thm}

\declaretheorem[name=Theorem,refname=Thm.]{theorem}
\declaretheorem[name=Lemma,sibling=theorem]{lemma}
\declaretheorem[name=Proposition,refname=Prop.,sibling=theorem]{proposition}
\declaretheorem[name=Remark]{remark}
\declaretheorem[name=Corollary,refname=Cor.,sibling=theorem]{corollary}
\declaretheorem[name=Definition,refname=Def.]{definition}
\declaretheorem[name=Conjecture,sibling=theorem]{conjecture}
\declaretheorem[name=Axiom]{axiom}
\declaretheorem[name=Assumption,refname=Asm.]{assumption}




\declaretheorem[name=Example]{example}



\def\sectionautorefname{Sec.}
\def\subsectionautorefname{Sec.}


\definecolor{dgreen}{rgb}{0.00,0.49,0.00}
\definecolor{dblue}{rgb}{0,0.08,0.75}
% \usepackage{hyperref}       % hyperlinks
% \RequirePackage[colorlinks,citecolor=green,urlcolor=blue,linkcolor=blue]{hyperref}
\hypersetup{
    colorlinks = true,
    citecolor=dgreen,
    urlcolor=dblue,
    linkcolor=dblue
}


\crefname{assumption}{Assumption}{Assumptions}
\crefname{equation}{}{}
\crefname{figure}{Fig.}{Figs.}
\crefname{table}{Tab.}{Tabs.}
\crefname{section}{Sec.}{Sec.}
\crefname{theorem}{Thm.}{Thm.}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Cor.}{Cor.}
\crefname{example}{Example}{Examples}
\crefname{remark}{Remark}{Remarks}
\crefname{algorithm}{Alg.}{Algorightms}

\crefname{appendix}{Appendix}{Appendices}
\crefname{subappendix}{Appendix}{Appendices}
\crefname{subsubappendix}{Appendix}{Appendices}







\usepackage{etoolbox}


\AfterEndEnvironment{restatable}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{theorem}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{remark}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{example}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{assumption}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{lemma}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{proof}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{corollary}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{proposition}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{definition}{\noindent\ignorespacesafterend}



%------ Names & Acronyms ---------
% \newcommand{\spmlTitle}{A Structured Prediction Approach for Conditional Meta-Learning}
% \newcommand{\paperTitle}{Few-Shot Classification by Meta Label Learning}

\newcommand{\paperTitle}{The Role of Global Labels in Few-Shot Classification and How to Infer Them}


%Few-Shot Classification by Meta Label Learning
%Reformulating FSL / as global MCC 
%The interplay Understating 
\newcommand{\fslong}{few-shot learning}
\newcommand{\fsl}{FSL}
\newcommand{\spml}{TASML}
\newcommand{\laml}{MeLa}
\newcommand{\spmlong}{Task-adaptive Structured Meta-Learning}
\newcommand{\preTrainFeat}{Pre-trained Features}
\newcommand{\lsmetal}{{\textsc{LS~Meta-Learn}}}
\newcommand{\imgnet}{\textsc{ImageNet}}
\newcommand{\mimg}{\textit{mini}\imgnet{}}
\newcommand{\timg}{\textit{tiered}\imgnet{}}
\newcommand{\cifar}{\textsc{CIFAR-FS}}
\newcommand{\leo}{{LEO}}
\newcommand{\sploss}{{\bigtriangleup}}
%---------------------------------

\newcommand{\queryn}{n_q}
\newcommand{\supportn}{n_s}

\newcommand{\msf}[1]{\mathsf{#1}}
\newcommand{\mbf}[1]{\mathbf{#1}}


\newcommand{\R}{{\mathbb{R}}}
\newcommand{\N}{{\mathbb{N}}}


\newcommand{\EE}{\mathbb{E}}
\newcommand{\Lagr}{\mathcal{L}}


\newcommand{\X}{{\mathcal{X}}}
\newcommand{\Y}{{\mathcal{Y}}}
\newcommand{\Z}{{\mathcal{Z}}}
\newcommand{\F}{{\mathcal{F}}}
\newcommand{\D}{{\mathcal{D}}}
\newcommand{\A}{{\mathcal{A}}}


\newcommand{\hh}{{\mathcal{H}}}
\newcommand{\G}{{\mathcal{G}}}

\newcommand{\hs}{{\textrm{HS}}}
\newcommand{\HS}{{\hs}}

\newcommand{\alg}{\textrm{Alg}}
\newcommand{\jointAlg}{T}

\newcommand{\condmetapar}{\tau}
\newcommand{\Condmetapar}{{\mathcal{T}}}
\newcommand{\Q}{\mathcal{Q}}

% \newcommand{\citep}{\cite}


\renewcommand{\paragraph}[1]{\noindent{\bfseries #1.}}

\newcommand{\gstar}{{g^*}}


\newcommand{\eqals}[1]{\begin{align*}#1\end{align*}}

\newcommand{\eqal}[1]{\begin{align}#1\end{align}}

\newcommand{\dtr}{S}
\newcommand{\dval}{Q}
\newcommand{\dm}{D_{\rm global}}
\newcommand{\Tau}{\mathcal{T}}
\newcommand{\embd}{\psi_{\theta}}

\providecommand{\scal}[2]{\left\langle{#1},{#2}\right\rangle}
\providecommand{\norb}[1]{\bigl\|{#1}\bigr\|}
\providecommand{\nor}[1]{\left\|{#1}\right\|}

\newcommand{\ridge}{w}

